Indiscriminate Data Poisoning Attacks on Pre-trained Feature Extractors

Machine learning models have achieved great success in supervised learning tasks for end-to-end training, which requires a large amount of labeled data that is not always feasible. Recently, many practitioners have shifted to self-supervised learning methods that utilize cheap unlabeled data to learn a general feature extractor via pre-training, which can be further applied to personalized downstream tasks by simply training an additional linear layer with limited labeled data. However, such a process may also raise concerns regarding data poisoning attacks. For instance, indiscriminate data poisoning attacks, which aim to decrease model utility by injecting a small number of poisoned data into the training set, pose a security risk to machine learning models, but have only been studied for end-to-end supervised learning. In this paper, we extend the exploration of the threat of indiscriminate attacks on downstream tasks that apply pre-trained feature extractors. Specifically, we propose two types of attacks: (1) the input space attacks, where we modify existing attacks to directly craft poisoned data in the input space. However, due to the difficulty of optimization under constraints, we further propose (2) the feature targeted attacks, where we mitigate the challenge with three stages, firstly acquiring target parameters for the linear head; secondly finding poisoned features by treating the learned feature representations as a dataset; and thirdly inverting the poisoned features back to the input space. Our experiments examine such attacks in popular downstream tasks of fine-tuning on the same dataset and transfer learning that considers domain adaptation. Empirical results reveal that transfer learning is more vulnerable to our attacks. Additionally, input space attacks are a strong threat if no countermeasures are posed, but are otherwise weaker than feature targeted attacks.

==> others.tex <==
\subsection{Is one point enough to poison a neural network?}
We inject a single large data point into the dataset ($m\cdot torch.ones$) -- it is used exactly once per epoch.

First of all, why do neural networks breakdown under large yet uniform points?

\blue{Update: }\textbf{For MNIST, this is because large points induce gradient explosion.} Show the graphs and output in Notion.

\blue{Update: } From the experiments,
\begin{enumerate}
    \item it is harder to poison one/two layer NNs than larger NNs
    \item larger NNs have lower gradient norms
    \item multiplying the existing magnitude by $10$, in these new experiments, lead to 10 times increase in gradient magnitude - across all architectures
\end{enumerate}

For CIFAR-10, the gradient seems to remain around the same regardless of the alpha. This is because the batch norm's running average is magnified. In table \ref{tab:batch-norm-mean}, we can see that only the very first batch norm layer has its mean magnified - after the first batch norm layer, data size go back to normal again.

It is also interesting to note that inserting a single data point (black/white image) within bounds ($\alpha = 0$) leads to > 4\% accuracy drop.

\begin{table*}[ht]
    \centering
    %\small
    \caption{Large data attack with one data point of different $\alpha$ on various architectures. Here we train the model for 20 epochs with torch.optim.SGD(params, lr=0.01, momentum=0.9) for MNIST, torch.optim.SGD(params, lr=0.1, momentum=0.9) for 50 epochs for cifar-10, and batch size=1000 for both}
    \label{tab:large-data}    
    %\scriptsize
    \setlength\tabcolsep{6pt}
   \begin{tabular}{lcccccccccc}
\toprule
\bf $\alpha$ & clean & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 \\

\midrule

\blue{Update: }MNIST LR & 91.93\% & 92.09\% & 92.06\% & 92.02\% & 91.96\% & 90.98\% & 74.74\% & 20.84\% & 9.58\%   \\
\blue{Update: }MNIST 2-layer NN & 95.46\% & 95.6\% & 95.52\% & 95.47\% & 95.39\% & 94.14\% & 83.41\% & 87.55\% & 30\%   \\
\blue{Update: }MNIST 3-layer NN & 96.19\% & 96.25\% & 96.17\% & 96.07\% & 96.32\% & 95.36\% & 11.35\% & 9.8\% & 9.8\%   \\
\blue{Update: }MNIST 4-layer NN & 96.55\% & 96.31\% & 96.35\% & 96.44\% & 96.34\% & 96.36\% & 9.8\% & 11.35\% & 9.8\%   \\
\blue{Update: }MNIST 5-layer NN & 96.6\% & 96.83\% & 96.74\% & 96.84\% & 96.61\% & 96.28\% & 9.8\% & 9.8\% & 9.8\%   \\
\vio{Re-ran: }MNIST 6-layer NN & 97.1\% & 97.06\% & 96.87\% & 96.92\% & 96.84\% & 96.96\% & 9.8\% & 9.8\% & 9.8\%   \\

\midrule

CIFAR-10 resnet-18 & 73.33\% & 68.54\% & 11.28\% & 10\% & 10\% & 10\% & 10\% & 10\% & 10\%   \\


\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[ht]
    \centering
    %\small
    \caption{Gradient l2 norm sum at 1st epoch, rounded to the nearest integer}
    \label{tab:large-data-grad}    
    %\scriptsize
    \setlength\tabcolsep{6pt}
   \begin{tabular}{lcccccccccc}
\toprule
\bf $\alpha$ &
 clean & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7  \\

\midrule

\blue{Update: }MNIST LR & 68 & 24 & 367 & 3839 & 39599 & 395981 & 3959799 & 19798990 & 395979808   \\
\blue{Update: }MNIST 2-layer NN & 86 & 23 & 275 & 2775 & 31831 & 323155 & 3422011 & 33410942 & 335293952   \\
\blue{Update: }MNIST 3-layer NN & 98 & 15 & 127 & 1986 & 11664 & 201186 & 2001911 & 19301012 & 187860384   \\
\blue{Update: }MNIST 4-layer NN & 68 & 9 & 69 & 1054 & 9822 & 106011 & 1101543 & 10109646 & 105003576   \\
\blue{Update: }MNIST 5-layer NN & 31 & 6 & 39 & 391 & 5149 & 54194 & 555733 & 5159212 & 55985016   \\
\vio{Re-ran: }MNIST 6-layer NN & 13 & 4 & 19 & 189 & 2275 & 25902 & 246657 & 2516816 & 28933478  \\

\midrule

CIFAR-10 resnet-18 & 382 & 4378 & 4387 & 5010 & 4562 & 4803 & 4169 & 4486 & 4400   \\


\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[ht]
    \centering
    %\small
    \caption{l2 norm of running (mean, variance) for various batch norm layers on CIFAR-10 resnet-18 after epoch 1}
    \label{tab:batch-norm-mean}    
    %\scriptsize
    \setlength\tabcolsep{6pt}
   \begin{tabular}{lcccccccccc}
\toprule
\bf $\alpha$ &
 clean & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7  \\

\midrule

First batch norm & 0.33 , 1.03 & 0.29 , 1.18 & 19.57 , 7.16 & 174.2 , 662.15 & 1753.34 , 57153.35 & - & - & - & -   \\
Second batch norm & 5.72 , 13.49 & 5.45 , 10.79 & 3.85 , 9.68 & 3.64 , 9.6 & 4.97 , 10.15 & - & - & - & -   \\
Third batch norm & 4.96 , 9.98  & 4.79 , 10.78 & 4.03 , 9.63 & 5.09 , 9.2 & 4.4 , 8.8 & - & - & - & -   \\
Last batch norm & 10.58 , 16.02  & 11.25 , 16.12 & 10.45 , 15.4 & 12.47 , 16.2 & 11.12 , 15.29 & - & - & - & -   \\


\bottomrule
\end{tabular}
\end{table*}



\subsection{How about ten points (injected in the same batch)?}
For MNIST, ten points instead of one naturally leads to the gradient multiplied by ten, and thus, we require alpha to be one magnitude lower. This is verified by the experiments in table \ref{tab:large-data-10}. Note that the gradients are of the same magnitude because they are the mean gradients--it needs to be multiplied by 10 to reflect the value of sum of the 10 gradients, which is indeed 10 times larger than before.

For CIFAR10, the injection of 10 times the number of points in the same batch lead to roughly 10\% accuracy drop for $\alpha = 0$. Note that this is actually within the clipped bounds of CIFAR-10 images.


\begin{table*}[ht]
    \centering
    %\small
    \caption{Large data attack with 10 data points, same params otherwise}
    \label{tab:large-data-10}    
    %\scriptsize
    \setlength\tabcolsep{6pt}
   \begin{tabular}{lcccccccccc}
\toprule
\bf $\alpha$ & clean & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 \\

\midrule
MNIST LR & \% & \% & \% & \% & \% & \% & \% & \% & \%   \\
MNIST 6-layer NN & 97.41\% & 96.91\% & 96.84\% & 96.87\% & 96.46\% & 9.8\% & 9.8\% & 9.8\% & 9.8\%   \\

\midrule

CIFAR-10 resnet-18 & 73.33\% & 63.6\% & 13.01\% & 10\% & 10\% & 10\% & 10\% & 10\% & 10\%   \\


\bottomrule
\end{tabular}
\end{table*}


\begin{table*}[ht]
    \centering
    %\small
    \caption{Mean gradient l2 norm sum at 1st epoch for 10 points}
    \label{tab:large-data-10-grad}    
    %\scriptsize
    \setlength\tabcolsep{6pt}
   \begin{tabular}{lcccccccccc}
\toprule
\bf $\alpha$ &
 clean & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7  \\

\midrule

MNIST LR &  &  &  &  &  &  &  &  &   \\
MNIST 6-layer NN & 13 & 216 & 1259 & 2118 & 2364 & 122670496 & nan & nan & nan  \\

\midrule

CIFAR-10 resnet-18 & 382 & 4068 & 4442 & 4194 & 4368 & 4409 & 4219 & 4869 & 4855   \\


\bottomrule
\end{tabular}
\end{table*}

\subsection{\blue{Update:} Can we get in-bound attacks to work with more points?}

On MNIST, since the gradients are accumulated, it would take $10^\alpha$ number of points of magnitude $1$ to achieve a single point of magnitude $10^\alpha$'s result. This is impractical: even for a 6-layer NN, we would need $10^5$ points for an $1000$ point batch. That is equivalent to $\epsilon = 10$.

On CIFAR10, it already works: 10 black images leads to a roughly 10\% accuracy drop.

\subsection{\blue{Update:} Can we get in-bound attacks \emph{that look like real images} to work?}
On MNIST, it is unlikely since we can't even get in-bound attacks to work.

\textbf{}{To do:} Can we somehow show that this is impossible theoretically? First show an image between -1 and 1 can only induce a gradient so large, then show a gradient needs to be at least a certain size to disturb the parameters enough to poison its accuracy.

\textbf{To do:} For CIFAR10, we might be able to.

\subsection{Gradient depends directly on the size of data point}

Take an simple example where we use the cross-entropy loss on a linear classifier. Suppose there are $c$ classes, let $(x, y)$ be a single input point and $w_c$ be the weight vector of class $c$. Then the loss is

$$
-\log(\frac{e^{x\cdot w_y}}{\sum_c e^{x\cdot w_c}}) = -x\cdot w_y + \log \sum_c e^{x\cdot w_c}
$$

We can calculate the derivative with respect to the weights:

$$
\frac{\partial L}{\partial w_y} = -x + \frac{1}{\sum_c e^{x\cdot w_c}} e^{x\cdot w_y}x = x(\frac{e^{x\cdot w_y}}{\sum_c e^{x\cdot w_c}} - 1)
$$

And for $y'\neq y$
$$
\frac{\partial L}{\partial w_{y'}} = \frac{1}{\sum_c e^{x\cdot w_c}} e^{x\cdot w_{y'}}x = x(\frac{e^{x\cdot w_{y'}}}{\sum_c e^{x\cdot w_c}})
$$

\textbf{Why large data poisoning works.} As x is scaled up, the soft-max constant goes to 1 if $w_y$ is the dominant weight (if $y = \argmax_c w_c\cdot x$), and 0 otherwise. However, when the model is just initialized, it is entirely possible for $w_y \cdot x$ to not be the dominant quantity, and thus the derivative scales up as $x$ scales up. So this gradient ends up dominating the rest.

\textbf{Why data poisoning within clipped range is difficult.} In any case, we can show that the gradients are bounded above because the magnitude of the constants that follow $x$ has absolute value at most 1. Poisoned data being bounded/clipped between $(-1, 1)$ as in the case of other MNIST data points means that each entry of the gradient is also bounded by 1. 

\textbf{How large do we need the poisoned gradient to be?} In our MNIST neural network experiments, the mean clean gradient is of l2-norm 13, so the unnormalized gradient is of size 13000. One might expect the poisoned gradient to beat this by a good margin to stop the model from learning. Indeed, when it occurs in $\alpha = 5$ for 1 point and $\alpha = 4$ for 10 points is where the poisoned gradient gets our optimizer to make a severely wrong step and go to infinity.

\subsection{Can we obtain a decoder for a given encoder?}
For this, I ran a basic autoencoder architecture on CIFAR-10 with BCELoss. The results are:

\begin{enumerate}
    \item If we can tune both the encoder and decoder from scratch, the reconstruction loss is 0.549.
    \item If we throw away the existing decoder, and run end-to-end training, we also achieve 0.549 loss.
    \item If we throw away the existing decoder, and fix the existing encoder, we also achieve 0.549 loss. 
\end{enumerate}

In this case, it is feasible to retrieve the decoder given the encoder.





==> sections/diff.tex <==
\onecolumn
\Large{\textbf{Summarization of changes made for major revision}}
\vskip 1cm
\normalsize

In the following file, we show the PDF differences by marking the changes we have made since the last revision in \textcolor{blue}{blue}. We first summarize all the changes here:
\vskip 0.3cm

\textbf{Required changes 1}: Cross-domain evaluation, including the extension to multimodal models, and a dataset with a high domain shift from pertaining. 
\vskip 0.1cm
\textbf{\vio{Answer:}} Note that we have addressed this concern in our last revision during the rebuttal, and we believe the reviewers find them adequate. Here we recall the changes we have made: (1) We have added the experiment on multimodal models (CLIP) in Appendix
B.2 and Table VI;
(2) We have added the experiment with a high domain shift from
pretraining (i.e., pretraining on ImageNet and transferring to
PatchCamelyon) in Appendix B.4 and Table VIII; 

\vskip 0.3cm

\textbf{Required changes 2}: Clarify the threat model and make clear that only availably attacks are considered and why (add more details about the knowledge and capability of the attacker).
\vskip 0.1cm
\textbf{\vio{Answer:}} We have added the following two paragraphs at the beginning of Section III.A, pages 3-4 on our threat model:


\begin{framed}
We first specify our \textbf{threat model}:
\begin{itemize}
    \item Knowledge of the attacker: the attacker has access to the training data, the target model (including its pre-trained weights), and the training procedure;
    \item Capability: the attacker can (actively or passively) inject a poisoned set to the training data; 
    \item Objective: given a pre-trained feature extractor, the objective of a downstream task and the corresponding training dataset, an adversary aims to construct a poisoned set to augment the clean training set, such that by training on the mixed dataset, the performance of the downstream task on the test set is reduced. 
\end{itemize}

Note that in this paper we only consider indiscriminate attacks. Another strong threat is the targeted attacks, where the knowledge of the attacker is expanded to some target test data, and the objective is to alter the prediction of them. The power of such attacks on pre-trained feature extractors has been studied and we refer interested readers to \cite{ShafahiHNSSDG18}. 
\end{framed}


\vskip 0.3cm

\textbf{Required changes 3}: Show how the poisoning performs on a classifier (e.g. take the layer before the classifier head as the feature layer to optimize) to compare the results.
\vskip 0.1cm
\textbf{\vio{Answer:}} This approach is included in Section IV.A (GC feature space attack) and is used as
an essential building block of our later attacks, and an important
baseline in Table I and Table II. We have added the following paragraph in Section V.B.2 on page 9 to further elaborate GC feature space attack and its intentions:




\begin{framed}
Note that we do not treat GC feature space attack as a viable attack (as injecting poisoned features may not be realistic), but as an essential building block and intermediate step for decoder inversion and feature matching. Additionally, our following results for GC feature space attack provide important information on how good a poisoned feature $\zeta$ can be (in terms of attack performance) and the difficulty of inverting them back to the input space.
\end{framed}

\textbf{Required changes 4}: Discuss how GC-input and Feature Matching can be compared/what are the differences.
\vskip 0.1cm
\textbf{\vio{Answer:}}  We have added the following paragraph in Section V.B.2 on pages 9-10 to further compare GC-input and feature matching attacks:




\begin{framed}
Moreover, we compare the best-performing input space attack (GC-input) and feature targeted attack (feature matching). Recall that both of these methods aim to solve the same constrained problem in \Cref{eq:gc_input}, where GC-input directly the constrained gradient canceling problem while the latter approach mitigates the difficulty of the constrained problem with the staged strategy in \Cref{eq:gc_input-relax}. We observe that the feature matching attack indeed helps with the optimization procedure and improves the attack effectiveness by a big margin (range from 3.80\% to 6.16\% for different $\epsilon_d$).
\end{framed}
